Quatro++: Robust Global Registration Exploiting Ground Segmentation for Loop Closing in LiDAR SLAM

Global registration is a fundamental task that estimates the relative pose between two viewpoints of 3D point clouds. However, there are two issues that degrade the performance of global registration in LiDAR SLAM: one is the sparsity issue and the other is degeneracy. The sparsity issue is caused by the sparse characteristics of the 3D point cloud measurements in a mechanically spinning LiDAR sensor. The degeneracy issue sometimes occurs because the outlier-rejection methods reject too many correspondences, leaving less than three inliers. These two issues have become more severe as the pose discrepancy between the two viewpoints of 3D point clouds becomes greater. To tackle these problems, we propose a robust global registration framework, called \textit{Quatro++}. Extending our previous work that solely focused on the global registration itself, we address the robust global registration in terms of the loop closing in LiDAR SLAM. To this end, ground segmentation is exploited to achieve robust global registration. Through the experiments, we demonstrate that our proposed method shows a higher success rate than the state-of-the-art global registration methods, overcoming the sparsity and degeneracy issues. In addition, we show that ground segmentation significantly helps to increase the success rate for the ground vehicles. Finally, we apply our proposed method to the loop closing module in LiDAR SLAM and confirm that the quality of the loop constraints is improved, showing more precise mapping results. Therefore, the experimental evidence corroborated the suitability of our method as an initial alignment in the loop closing. Our code is available at https://quatro-plusplus.github.io.

==> contents/quatro_pp_table.tex <==

\begingroup
\begin{table}[t!]
	\centering
	\captionsetup{font=footnotesize}
	\caption{Success rate {(unit: \%) for situations where distance is between 9$\sim$12 m away under the loop closing condition} in the KITTI dataset~\citep{geiger2012kitticvpr}. The registration result was considered successful when the transition
	{and rotation errors were not larger than 2~m and 10$^\circ$, respectively}. The criteria {were set based on~\cite{kim2019gp}}: a pose difference sufficient for the local registration to allow the estimate to converge toward global minima.}
	\setlength{\tabcolsep}{5pt}
	\begin{tabular}{l|cccccc}
	
	\toprule \midrule
	Method & \texttt{00} & \texttt{02} & \texttt{05} & \texttt{06} & \texttt{07} &  \texttt{08}  \\ \midrule
	RANSAC & 10.7 & 9.6 & 11.15 & 4.4 & 18.4 & 10.0 \\
	FGR  & 46.0 & 21.2 & 47.8 & 59.2 & 41.2 & 15.9  \\
 	TEASER++~ & 84.4 & 70.7 & 94.1 & 96.8 & 97.7 & 98.7  \\
 	Quatro & 84.3 & 71.3 & 93.7 & 97.7 & 95.2 & 98.7  \\
 	Quatro++ & \textbf{87.1} &\textbf{ 90.8} & \textbf{98.5} & \textbf{100.0} & \textbf{98.0} & \textbf{98.9}  \\\midrule\bottomrule
	\end{tabular}
	\label{table:success_rate}
	\vspace{-0.3cm}
\end{table}
\endgroup
